Modified (hyper-)viscosity for coarse-resolution ocean models

We present a simple parameterization for coarse-resolution ocean models. To replace computationally expensive high-resolution ocean models, we develop a computationally cheap parameterization for coarse-resolution models based solely on the modification of the viscosity term in advection equations. It is meant to reproduce the mean quantities like pressure, velocity, or vorticity computed from a high-resolution reference solution or using observations. We test this new parameterization on a double-gyre quasi-geostrophic model in the eddy-permitting regime. Our results show that the proposed scheme improves significantly the energy statistics and the intrinsic variability on the coarse mesh. This method shall serve as a deterministic basis model for coarse-resolution stochastic parameterizations in future works.

==> stuod_proc(9)/ref.tex <==
\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution

\bibitem{arakawa1981potential} Arakawa, Akio and Lamb, Vivian R (1981), A potential enstrophy and energy conserving scheme for the shallow water equations. Monthly Weather Review 109:18--36.


\bibitem{fox2008can} Fox-Kemper, B and Menemenlis, D (2008), Can large eddy simulation techniques improve mesoscale rich ocean models?. Washington DC American Geophysical Union Geophysical Monograph Series 177:319--337.

\bibitem{fox2014principles}  Fox-Kemper, B and Bachman, S and Pearson, B and Reckinger, S (2014), Principles and advances in subgrid modelling for eddy-rich simulations. CLIVAR Exchanges No. 65, Vol. 19, No. 2.

\bibitem{frisch2008hyperviscosity} Frisch, Uriel and Kurien, Susan and Pandit, Rahul and Pauls, Walter and Ray, Samriddhi Sankar and Wirth, Achim and Zhu, Jian-Zhou (2008), Hyperviscosity, Galerkin truncation, and bottlenecks in turbulence. Physical review letters 101:144501.

\bibitem{griffies2000biharmonic} Griffies, Stephen M and Hallberg, Robert W (2000), Biharmonic friction with a Smagorinsky-like viscosity for use in large-scale eddy-permitting ocean models. Monthly Weather Review 128:2935--2946.

\bibitem{hogg2003quasi} Hogg, Andrew Mc C and Dewar, William K and Killworth, Peter D and Blundell, Jeffrey R (2003), A quasi-geostrophic coupled model (Q-GCM). Monthly Weather Review 131:2261--2278.

\bibitem{hogg2005mechanisms} Hogg, Andrew Mc C and Killworth, Peter D and Blundell, Jeffrey R and Dewar, William K (2005), Mechanisms of decadal variability of the wind-driven ocean circulation. Journal of physical oceanography 35:512--531.

\bibitem{hogg2014formulation} Hogg, AM and Blundell, JR and Dewar, WK and Killworth, PD (2014), Formulation and users’ guide for Q-GCM, \href{http://q-gcm.org/downloads/q-gcm-v1.5.0.pdf}{http://q-gcm.org/downloads/q-gcm-v1.5.0.pdf}.

\bibitem{holm1998hamilton} Darryl D. Holm, Vladimir Zeitlin (1998), Hamilton’s principle for quasigeostrophic motion. Physics of fluids 10(4):800--806.

\bibitem{jansen2014parameterizing} Jansen, Malte F and Held, Isaac M (2014), Parameterizing subgrid-scale eddy effects using energetically consistent backscatter. Ocean Modelling 80:36--48.


% not used
% \bibitem{leith1990stochastic} Leith, CE (1990), Stochastic backscatter in a subgrid-scale model: Plane shear mixing layer. Physics of Fluids A: Fluid Dynamics 2:297--299.

\bibitem{leith1996stochastic} Leith, CE (1996), Stochastic models of chaotic     systems. Physica D: Nonlinear Phenomena 98:481--491.

\bibitem{memin2014fluid} M{\'e}min, Etienne (2014), Fluid flow dynamics under location uncertainty. Geophysical \& Astrophysical Fluid Dynamics 108:119--146.

\bibitem{paszke2019pytorch} Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others (2019), Pytorch: An imperative style, high-performance deep learning library. Advances in neural information processing systems 32:8026--8037.

\bibitem{ryzhov2020data} Ryzhov, EA and Kondrashov, D and Agarwal, N and McWilliams, JC and Berloff, P (2020), On data-driven     induction of the low-frequency variability in a coarse-resolution ocean model. Ocean Modelling 153:101664


\bibitem{roullet2021fast} Roullet, Guillaume and Gaillard, Tugdual (2021), A Fast Monotone Discretization of the Rotating Shallow Water Equations, ESSOAR/JAMES.

\bibitem{shevchenko2015multi} Shevchenko, IV and Berloff, PS (2015), Multi-layer quasi-geostrophic ocean dynamics in eddy-resolving regimes. Ocean Modelling 94:1--14.


\bibitem{smagorinsky1963general} Smagorinsky J. (1963), General circulation experiments with the primitive equations. Monthly weather review 91.3:99-164.

\bibitem{Vallis2017atmos} Vallis, G. K. (2017), Atmospheric and oceanic fluid dynamics: fundamentals and large-scale circulation. Cambridge University Press.
%
\end{thebibliography}
